Online Reciprocal Recommendation with Theoretical Performance Guarantees

A reciprocal recommendation problem is one where the goal of learning is not just to predict a user's preference towards a passive item (e.g., a book), but to recommend the targeted user on one side another user from the other side such that a mutual interest between the two exists. The problem thus is sharply different from the more traditional items-to-users recommendation, since a good match requires meeting the preferences of both users. We initiate a rigorous theoretical investigation of the reciprocal recommendation task in a specific framework of sequential learning. We point out general limitations, formulate reasonable assumptions enabling effective learning and, under these assumptions, we design and analyze a computationally efficient algorithm that uncovers mutual likes at a pace comparable to those achieved by a clearvoyant algorithm knowing all user preferences in advance. Finally, we validate our algorithm against synthetic and real-world datasets, showing improved empirical performance over simple baselines.

==> contributions.tex <==
\section{Main contributions and results}

The main contributions and results of this work can be summarized as follows:

\begin{itemize}

\item We take a first step toward a rigorous formalization of online reciprocal recommendation problems, where the user features are not available and can be seen therefore as encoded in the user feedback. This choice can be motivated in several ways, as explained in the introduction. For instance, in many important practical scenarios the features associated
with some users are not always acquirable (or reliable) and, in addition, may face severe scaling issues.  
Furthermore, the use of personal features, in some contexts may generate privacy issues related to sensitive data of the user profiles. %Finally, given the massive user data for the related real-world applications, there is need to help users filtering the most relevant information in the abundant pool of choices. 

\item In the adversarial setting, we provide an upper bound for the number of pairs of users that can be matched by {\em any} algorithm during $T$ rounds, and show its tightness by describing and analysing a simple optimal matching strategy. This quantifies therefore the performance that can be achieved when there are no constraints on the edge sign assignment in the input.

\item We propose a natural model based on hidden user preference/description features, showing that its assumptions in the generation process of edge sign assignments appear to be necessary to learn which pairs of users match. With this operational framework it is possible to address reciprocal recommendation problems from several different perspectives, design new algorithms and compare their performance from a quantitive point of view. The proposed model is general and flexible enough to capture the complexity of real-world instances of this problem. At the same time, through the interplay between the combinatorial constraints of designing matchmakers and the adversarial strategies, it also provides a clear definition of the learning task within this context. Finally, as explained in Section~\ref{s:refinements}, it is possible to refine and extend the model in several interesting directions. 

\item We describe an algorithm, 
%that we called \smi, 
able to exploit the correlation of match pairs generated according to the model we proposed. We analyze this matching strategy showing that, for {\em any} input, it is optimal up to a constant factor when the total number of rounds and matches is not too small (see Theorem~\ref{th:smileMatchMequalMstar}). 

\item In Theorem~\ref{th:smileTimeNeeded} we quantify to what extent the number of rounds required by \smi\ to achieve an optimal performance is necessary.

\item In the proof of Theorem~\ref{th:smileCompComplexity}, we describe step by step how to combine and use some suitable data structures obtaining a computationally efficient implementation of \smi. 

\end{itemize}

==> listofitems.tex <==
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                     {1.53}                               %
%                                                                    %
\def\loidate                  {2018/03/13}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Author     : Christian Tellechea, Steven B. Segletes
% Status     : Maintained
% Maintainer : Christian Tellechea
% Email      : unbonpetit@netc.fr
%              steven.b.segletes.civ@mail.mil
% Package URL: https://www.ctan.org/pkg/listofitems
% Bug tracker: https://framagit.org/unbonpetit/listofitems/issues
% Repository : https://framagit.org/unbonpetit/listofitems/tree/master
% Copyright  : Christian Tellechea 2017-2018
% Licence    : Released under the LaTeX Project Public License v1.3c
%              or later, see http://www.latex-project.org/lppl.txt
% Files      : 1) listofitems.tex
%              2) listofitems.sty
%              3) listofitems-fr.tex
%              4) listofitems-fr.pdf
%              5) listofitems-en.tex
%              6) listofitems-en.pdf
%              7) README
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\ProvidesPackage\else
	\immediate\write -1 {%
	Package: \loidate\space v\loiver\space Grab items in lists using user-specified sep char (CT)}%
\fi

\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% gestion des erreurs %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% v\'erification de la pr`'esence de etex %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup
\edef\__tempa{\meaning\eTeXversion}\edef\__tempb{\string\eTeXversion}%
\ifx\__tempa\__tempb
	\endgroup
\else
	\endgroup
	\loi_error{You are not using an eTeX engine, listofitems cannot work.}%
	\expandafter\loi_restorecatcode\expandafter\endinput
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---- macros de d\'eveloppement et de manipulation d'arguments
\chardef\loi_stop=0
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_exparg#1#2{\expandafter\loi_exparg_i\expandafter{#2}{#1}}% \loi_exparg{<a>}{<b>} devient <a>{<*b>}
\long\def\loi_exparg_i#1#2{#2{#1}}
\long\def\loi_expafter#1#2{\expandafter\loi_expafter_i\expandafter{#2}{#1}}% \loi_expafter{<a>}{<b>} devient <a><*b>
\long\def\loi_expafter_i#1#2{#2#1}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\loi_argcsname_i{#1}}
\def\loi_argcsname_i#1#2{\loi_expafter{#1}{\csname#2\endcsname}}

%--- macros de test
\long\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_i{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_i}
\long\def\loi_ifprimitive#1{\edef\loi_tempa{\meaning#1}\edef\loi_tempb{\string#1}\loi_ifx{\loi_tempa\loi_tempb}}
\long\def\loi_ifcs#1{% #1 est-il une sc (n'\'etant pas une primitive) ?
	\loi_ifempty{#1}
		\loi_second% si #1 est vide, faux
		{\loi_ifspacefirst{#1}
			\loi_second% si espace en 1er, faux
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\begingroup \escapechar`\_
					\if\expandafter\loi_firsttonil\detokenize{#1}\_nil\expandafter\loi_firsttonil\string\relax\_nil
						\loi_ifprimitive{#1}
							{\endgroup\expandafter\loi_second}
							{\endgroup\expandafter\loi_first}%
					\else
						\endgroup\expandafter\loi_second
					\fi
				}
				\loi_second% si plusieurs tokens, faux
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }\loi_second\loi_first}

%--- macro de type for
%      Voir codes 150 \`a 155 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 175 \`a 184 du livre "Apprendre \`a programmer en TeX"
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}\edef\loi_sgncmp{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
	\expandafter\loi_fornum_i\csname loi_fornum_\string#1\expandafter\endcsname\expandafter{\number\numexpr#3\expandafter}\loi_sgncmp#1%
}
\long\def\loi_fornum_i#1#2#3#4#5#6{\def#1{\unless\ifnum#5#3#2\relax\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}\fi}#1}

%--- macros retirant les espaces extr\^emes
%      Voir codes 320 \`a 324 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 339 \`a 343 de "Apprendre \`a programmer en TeX"
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_i\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_i#1 #2\_nil{\loi_ifempty{#1}}
\expandafter\def\expandafter\loi_gobspace\space{}
\def\loi_removefirstspaces{\romannumeral\loi_removefirstspaces_i}
\long\def\loi_removefirstspaces_i#1{\loi_ifspacefirst{#1}{\expandafter\loi_removefirstspaces_i\expandafter{\loi_gobspace#1}}{\loi_stop#1}}
\edef\loi_restorezerocatcode{\catcode0=\number\catcode0 \relax}
\catcode0 12
\long\def\loi_removelastspaces#1{\romannumeral\loi_removelastspaces_i#1^^00 ^^00\_nil}
\long\def\loi_removelastspaces_i#1 ^^00{\loi_removelastspaces_ii#1^^00}
\long\def\loi_removelastspaces_ii#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_i#1^^00 ^^00\_nil}{\loi_stop#1}}
\loi_restorezerocatcode
\long\def\loi_removeextremespaces#1{% #1=texte o\`u les espaces extr\^emes sont retir\'es
	\romannumeral\expandafter\expandafter\expandafter\loi_removelastspaces\expandafter\expandafter\expandafter
	{\expandafter\expandafter\expandafter\loi_stop\loi_removefirstspaces{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_i}
\def\setsepchar_i{\loi_ifx{[\loi_nxttok}\setsepchar_ii{\setsepchar_ii[/]}}
\long\def\setsepchar_ii[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_ii[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % r\'einitaliser niveau initial \`a 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_iv1{,}%
			}
			{\readlist_iv1{#2}}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de s\'eparation
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2#3{% #1=macroname  #2=liste d'index  #3=profondeur max --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{\loi_stop{}{}}
		{\loi_normalizeindex_i1{}{#3}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_i#1#2#3#4#5,{% #1=compteur de profondeur #2=index pr\'ec\'edents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_iii#2\loi_quark}% supprimer la derni\`ere virgule
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}}% si profondeur trop grande
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_ii{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_ii#1#2#3{\loi_exparg\loi_normalizeindex_i{\number\numexpr#2+1}{#3#1,}}% #1=index \`a rajouter  #2=compteur de profondeur #3=index pr\'ec\'edents
\def\loi_normalizeindex_iii#1,\loi_quark{\loi_stop{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_i{#1},}\loi_invalidindex_i{#1}{#2}}
\def\loi_invalidindex_i#1#2{\loi_invalidindex_ii#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_ii#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{\loi_stop{#1[#3]#2}{#3}}% #4= index ignor\'es

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{\let\loi_def\gdef\let\loi_edef\xdef\def\loi_let{\global\let}\readlist_o}%
\def\readlist{\let\loi_def\def\let\loi_edef\edef\let\loi_let\let\readlist_o}
\def\readlist_o{%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\long\def\readlist_i#1#2{% #1=macro stockant les \'el\'ements  #2=liste des \'el\'ements
	\loi_ifcs{#2}
		{\loi_exparg{\readlist_i#1}{#2}}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_argcsname\loi_let{\loi_listname nest}\nestdepth
		\loi_argcsname\loi_def{\loi_listname[]}{#2}% la liste enti\`ere
		\loi_argcsname\loi_def{\loi_listname sep[]}{}% s\'eparateur vide
		\loi_ifempty{#2}
			{\loi_def#1[##1]{}%
			\loi_argcsname\loi_def{\loi_listname len}{0}\loi_argcsname\loi_def{\loi_listname len[0]}{0}%
			\loi_error{Empty list ignored, nothing to do}%
			}
			{\loi_edef#1[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname}}%
			\loi_argcsname\loi_edef{\loi_listname sep}[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname sep}}%
			\readlist_ii{#2}%
			\loi_argcsname\loi_argcsname\loi_let{\loi_listname len}{\loi_listname len[0]}% longueur du niveau 0
			}%
		}%
}
\def\loi_auxmacrolistitem#1#2#3{%
	\expandafter\expandafter\expandafter\loi_stop\csname#3[#2]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}
\def\readlist_ii{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_iii\loi_currentsep||\_nil
}
\long\def\readlist_iii#1||#2\_nil#3{\readlist_iv1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un \'el\'ement vide pour le test ifempty ci dessous
\long\def\readlist_iv#1#2{% #1=compteur d'index  #2=liste d'\'el\'ements \`a examiner
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\loi_argcsname\loi_let{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname\number\numexpr#1-1\relax]}\empty% le dernier <sep> est <vide> ##NEW v1.52
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafter{\readlist_vi{#2}{}}\loi_currentsep||\loi_quark||#2\_nil{#1}}% aller isoler le 1er item
}
\long\def\readlist_v#1#2{\readlist_vi{#2}{}#1||\loi_quark||#2\_nil}% #1=liste s\'eparateurs (s\'ep=||)  #2=chaine de tokens
\long\def\readlist_vi#1#2#3||{% #1=liste restante   #2=dernier <sep utile>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}
		{\loi_ifempty{#2}% si #1 vide, aucun <sep utile> n'a \'et\'e trouv\'e, il reste \`a lire "<liste compl\`ete>\_nil"
			{\long\def\readlist_vii##1\_nil##2{\loi_exparg{\readlist_ix{##2}{}}{\loi_gobarg##1}{#2}}}% ##2=compteur d'index
			{\long\def\readlist_vii##1#2{\loi_exparg\readlist_viii{\loi_gobarg##1}\relax}%
			\long\def\readlist_viii##1##2\_nil##3{\loi_exparg{\readlist_ix{##3}}{\loi_gobarg##2}{##1}{#2}}% ##3=compteur d'index
			}%
		\readlist_vii\relax% le \relax meuble l'argument d\'elimit\'e
		}
		{\long\def\readlist_vii##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_vi{#1}{#2}}% recommencer avec le m\^eme <sep utile>
				{\loi_exparg\readlist_vi{\loi_gobarg##1#3}{#3}}% sinon raccourcir <liste restante> et <sep courant>:=<sep utile>% ##BUGFIX v1.53
			}%
		\readlist_vii\relax#1#3\_nil% ##BUGFIX v1.53
		}%
}
\long\def\readlist_ix#1#2#3{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extr\^emes
		{\loi_exparg{\loi_exparg{\readlist_x{#1}{#2}}}{\loi_removeextremespaces{#3}}}% red\'efinir l'\'el\'ement courant
		{\readlist_x{#1}{#2}{#3}}%
}
\long\def\readlist_x#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant   #4=sep utilis\'e
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_iv{#1}{#2}}% si l'on n'ignore pas les \'el\'ements vides :
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation de l'item ctuel \`a la macro
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel \`a la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_ii{#3}% recommencer avec l'\'el\'ement courant
			}
			{}%
		\loi_exparg\readlist_iv{\number\numexpr#1+1}{#2}% puis chercher l'\'el\'ement suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\romannumeral\loi_ifempty{#2}
		{\expandafter\expandafter\expandafter\loi_stop\csname\loi_macroname#1len[0]\endcsname}
		{\loi_exparg\listlen_i{\romannumeral-`\.\loi_macroname#1}{#2}}%
}
\def\listlen_i#1#2{% #1=macro name   #2=index non normalis\'e    prendre <profondeur max-1>
	\loi_exparg{\expandafter\listlen_ii\romannumeral\loi_normalizeindex{#1}{#2}}{\number\numexpr\csname#1nest\endcsname-1}{#1}%
}
\def\listlen_ii#1#2#3{% #1=err   #2=index normalis\'e  #3=macroname
	\expandafter\expandafter\expandafter\loi_stop\csname#3len[#2,0]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_i{\noexpand\foreachitem_iii\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_ii
}
\def\foreachitem_ii{\loi_ifx{\loi_nxttok[}\foreachitem_i{\foreachitem_i[]}}
\def\foreachitem_iii#1#2#3[#4]{% prendre <profondeur max-1>
	\loi_exparg{\expandafter\foreachitem_iv\romannumeral\loi_normalizeindex{#3}{#4}}{\number\numexpr\csname#3nest\endcsname-1}#1{#2}{#3}%
}
\def\foreachitem_iv#1#2{\loi_ifempty{#2}{\foreachitem_v{#1}{}}{\foreachitem_v{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_v#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associ\'e  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_i}{\let\showitems_cmd\loi_identity\showitems_i}}
\def\showitems_i#1{\def\showitems_ii{\showitems_iv#1}\futurelet\loi_nxttok\showitems_iii}
\def\showitems_iii{\loi_ifx{\loi_nxttok[}\showitems_ii{\showitems_ii[]}}
\def\showitems_iv#1[#2]{\foreachitem\showitems_iter\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_iter}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % r\'eglages identiques \`a LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir codes 251 \`a 254 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
		\hbox{% et pages 271 \`a 274 de "Apprendre \`a programmer en TeX"
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par d\'efaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}{\global\let}%
}
\def\itemtomacro_i#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% r\'eglages par d\'efaut %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\setsepchar{,}
\reademptyitems

\loi_restorecatcode
\endinput

######################################################################
#                             Historique                             #
######################################################################

v1.0  19/8/2016
  - Premi\`ere version publique

v1.1  01/09/2016
  - Stockage des s\'eparateurs dans <macrolist>sep
  - bug corrig\'e dans \loi_restorecatcode

v1.2  22/10/2016
  - macros \greadlist et \gitemtomacro pour la globalit\'e

v1.3  18/11/2016
  - bugs corrig\'es dans la gestion de la globalit\'e

v1.4  05/10/2017
  - test \loi_ifprimitive ajout\'e au test \loi_ifcs
  - suppression de \loi_expafternil, cr\'eation de \loi_expafter,
    modification de \loi_argcsname
  - correction d'un bug : \setsepchar{\par} ne provoque plus
    d'erreur. \loi_ifnum devient \long

v1.5  06/10/2017
  - correction d'un bug dans \loi_ifcs

v1.51 24/10/2017
  - correction d'un bug dans \loi_ifcs

v1.52 13/01/2018
  - le dernier s\'eparateur est <vide>

v1.53 13/03/2018
  - correction d'un bug dans \readlist_vii

==> oldVersionLemmas.tex <==
\section{Lemmas used in previous versions of the draft}
\label{as:oldLemmas}
These lemmas can be seen as results for generalized versions of the Coupon Collector's problem. The former is part of this draft and deals with nonuniform probability distributions. The latter, due to Erdos and Renyi 
[\textit{cite}], provides tail estimates of the Coupon Collector generalization of Donald J. Newman and Lawrence Shepp [\textit{cite}].

\begin{lemma}\label{le:nonuniformCC}
We have a sequence $c_1, c_2, \ldots c_n$ of $n$ coupons associated with probabilities $p_1, p_2, \ldots, p_n$ respectively, such that $\sum_{i=1}^n p_i=1$.
In an online fashion, at each time step we select one coupon randomly with replacement according to the discrete distribution defined by the above set of probabilities $p_i$ for all $i \in [n]$. 
Then, for any value $z\ge 1$, the %expected 
%\footnote{\textit{\color{ForestGreen} \textbf{FV}: I am sure it is easy to generalize this lemma having a results which holds with high probability.}}
sum of the probabilities associated with the coupons that we collected during
$2z\, n \log(n)$ steps is bounded from below w.h.p.~%\footnote{\textit{\color{ForestGreen} \textbf{FV}: The terminology \enquote{w.h.p.} used in this draft will be replaced by \enquote{with probability at least $(1-\delta)$...}.}} 
 by $1-\frac{1}{z}$.
\end{lemma}

\begin{proof}\textit{[Sketch]}
The proof basically involves computing the sum of the expected values of geometric distributions, as in the well known proof of the standard (uniform) Coupon Collector problem, where one looks for the expected number of steps necessary to collect all the $n$ coupons. Let $p_{\pi(1)}, p_{\pi(2)}, \ldots, p_{\pi(n)}$ be a permutation of the sequence $p_1, p_2, \ldots, p_n$ such that $p_{\pi(i+1)} \le p_{\pi(i)}$ for all $i \in [n-1]$. In this descreasing sequence, let $p_{\pi(k)}$ be the smallest probability greater than or equal to $\frac{1}{z\,n}$. Thus we have 
$\sum_{k<i\le n} p_{\pi(i)}\le\frac{1}{z}$.
Now, let $S_k$ be the coupon subsequence $c_{\pi(1)}, c_{\pi(2)}, \ldots, c_{\pi(k)}$. Since the associated probability subsequence is decreasing, collecting the last coupon in $S_k$ requires in expectation at most $p_{\pi(k)}^{-1}$ time steps, collecting the last but one coupon in $S_k$ requires in expectation at most $(2\,p_{\pi(k)})^{-1}$ time steps, and so on until the first coupon in $S_k$, which requires in expectation at most $(k\,p_{\pi(k)})^{-1}$ time steps. Bounding from above the $k$-th partial sum of the harmonic series by $\log(n)$, we have that the sum of these expected values is at most $z\,n\log(n)$. Finally, the number of time steps required to obtain the same result w.h.p. can be found by applying a Union Bound as in the standard (uniform) Coupon Collector problem.
\end{proof}

\begin{lemma}\label{le:mcopiesCC}
Given $n$ coupons, we select one coupon {\em uniformly} at random with replacement at each time step, in an online fashion. Let $T_m$ be the first time $m$ copies of each coupon are collected. Then we have
\[
\Pr(T_m < n \log n + (m-1)n \log\log n+c\,n)\rightarrow
\exp\left(\frac{-\exp(-c)}{(m-1)!}\right)
\]
when $n$ goes to infinity.
\end{lemma}

==> omniscentMatchmaker.tex <==
\section{The Omniscient Matchmaker}\label{s:omni}

In this section we briefly describe a method that will be used as a \enquote{yardstick} comparison to measure the algorithmic performance in this framework, although it works with the help of a powerful oracle. The use of this comparison performance is necessary because, when $\degree_{\scM}(u) > \frac{T}{n}$ for some user $u$, no algorithm will be able to find all $M$ matches, since steps $1_B$ and $1_G$ entail that each user will be served $\frac{T}{n}$ in expectation, and the distribution of the number of times each user will be selected at step $1_B$ and $1_G$ concentrates around the mean value $\frac{T}{n}$.



We define the {\em Omniscient Matchmaker} as an {\em optimal} strategy based on the knowledge of \textbf{(i)} the value of $s(b,g)$ and $s(g,b)$ for all boys $b \in B$ and $g \in G$, and \textbf{(ii)} the whole ordered sequence of $T$ boys and $T$ girls selected respectively in step $2_B$ and $2_G$ during the sequence of all $T$ rounds. By writing \enquote{optimal}, we mean that, based on this information, the Omniscient Matchmaker operates as an algorithm maximising the number of matches found in $T$ rounds among 
{\em all} the $n^{2T}$ possible selections that can be made during $T$ rounds at step $2_B$ and $2_G$.

For the sake of completeness, we describe a method to implement this algorithm exploiting this information. Let $t(b)$ and $t(g)$ be the number of times boy $b$ and girl $g$ are selected during the $T$ rounds.
Knowing the above information \textbf{(i)} and \textbf{(ii)}, the Omniscient Matchmaker could be implemented with a slight modification of the Ford-Fulkerson algorithm for the Maximum Flow problem used for finding a Maximum Bipartite Matching. The matching graph $\scM$, known because of \textbf{(i)}, is transformed into a flow network, with two extra nodes: a source node $\widetilde{s}$, connected directly with all the boy nodes (from $\widetilde{s}$ to $B$), and a target node $\widetilde{t}$, connected directly with all girls (from $G$ to $\widetilde{t}$). If the weight of each direct edge $(\widetilde{s},b)$ for all $b \in B$ and 
$(g,\widetilde{t})$ for all $g \in G$ is set to $t(b)$ and 
$t(g)$ respectively, it is easy to see we obtain an optimal algorithm exploiting information \textbf{(i)} and \textbf{(ii)}. 

The above implementation description might simplify a comparison between the performance of any algorithm and the matches realized by this matchmaker that, as we said, we use as a performance yardstick comparison for this problem.

\medskip

We denote by $M^*_T$ the total number of users matched by this the Omniscient Matchmaker during $T$ rounds. 

\smallskip

Clearly, in general there is no algorithm capable to achieve this performance without exploiting information \textbf{(i)} and \textbf{(ii)}.
In fact, it is immediate to see that, when $\scM$ is a  uniformly random bipartite graph, the expected number of matches of any algorithm is always equal to 
$\scO\left(\frac{T}{n^2}M\right)$, whereas if $\degree_{\scM}(u) \le \frac{T}{n}$ for all users $u$, as $n$ approaches infinity, $\E M^*_T$ is equal to $\Theta(M)$  even with such adversarial random matching graph. 


More precisely, defining the quantity 
\[
\Delta(\scM,T)\defeq\sum_{u\in V}\max\left(\degree_{\scM}(u) - \frac{T}{n}, 0\right)~,
\] 
and taking into account that the number of times each user is selected at step $1_B$ and $1_G$ is modelled by a binomial distribution $B(T,n^{-1})$, we immediately derives the following fact. 

\begin{fact} The expected number $\E M^*_T$ of users matched by the Omniscient Matchmaker, is equal to 
$\Theta\left(\frac{M}{1+\Delta(\scM,T)}\right)$ when $n$ goes to infinity. 
\end{fact} 

Hence, when $\Delta(\scM,T)=\Theta(1)$, we have $\E M^*_T=\Theta(M)$.
Note that if $\degree_{\scM}(u) \le \frac{T}{n}$ for all users $u$, we have $\Delta(\scM,T)=0$.

\smallskip

%Finally, it is also easy to verify that, 
%a simple sufficient condition yielding $M^*_T=M$ w.h.p.~when $n$ goes to infinity, is 
%$T=\omega(n\log(n)\log\log(n))$ and $\max_{u\in V}\degree_{\scM}(u)=\scO\left(\frac{T}{n\log\log n}\right)$.


==> optimalAdversarialAlgorithm.tex <==
\section{An optimal algorithm for the adversarial setting}

We start this section pointing out that, performing the user selection always uniformly at random at each step $2_B$ and $2_G$, results in a highly suboptimal matching strategy. In fact we will be able to compare the expected number of matches found by this strategy with the performance of an optimal algorithm we propose for the adversarial setting, and verify that the ratio of the expected number of matches found by the two algorithms is equal to $\frac{T}{n^2}$. 

Let \uromm~(Uniformly Randomized Online MatchMaker) be the algorithm that simply selects uniformly at random a girl in $G$ and a boy in $B$ at each step $2_B$ and $2_G$ respectively. 

\begin{theorem}\label{th:urommLB}
Given any input graph $\scG(B,G,E,s)$, 
%if $T-n=\Omega(n)$ and $T\le n^2$, 
%then 
the expected number of matches found by 
%the algorithms 
%\idom\ and 
\uromm\ satisfies: 
\[
%\E M_T(\idom)=\Theta\left(
\E M_T(\uromm)
%\right)
=\Theta\left(\frac{T^2}{n^4}M\right)~.
\]
\end{theorem}



\bigskip

We now present an algorithm, called \om~(Oblivious Online MatchMaker), and prove it is optimal when no assumption is made about the sign assignment to the edges of the input graph. The general idea is to develop a strategy able to select $\Theta(T)$ pairs of reciprocal edges uniformly at random from $E_r$. We recall that $E_r$ is the set of {\em all} reciprocal edges between $B$ and $G$. Such an algorithm guarantees that the expected number of matches achieved is equal to $\Theta\left(\frac{T}{n^2}M\right)$, where the expectation is taken over the random choice of the $\Theta(T)$ pairs of reciprocal edges selected. In fact, each match must necessarily be a pair of reciprocal edges and will be selected this way with probability equal to $\frac{T}{n^2}$ up to a constant factor. In the description of matchmaking algorithms, according to the problem protocol of Section~\ref{s:protocol}, we only provide the two actions made by the learner, i.e. 
steps $2_B$ and $2_G$.

\begin{algorithm}
    \SetKwInOut{Input}{\scriptsize{$\triangleright$ INPUT}}
    \SetKwInOut{Step}{$\bullet$ Step}
    	\SetKwBlock{BeginSelectB}{\textbf{$\bullet$ Step 2$_{\bB}$}}{end}
	\SetKwBlock{BeginSelectG}{\textbf{$\bullet$ Step 2$_{\bG}$}}{end}
    \Input{User sets $B$ and $G$}
    \vspace{0.3cm}
    \textbf{At each round $t$:}\\
    \vspace{0.3cm}%
%    \Step{\textbf{2$_{\bB}$}}
\BeginSelectB{
	Select $g$ uniformly at random from $G$\;  
	}
    \vspace{0.3cm}
    %
%    \Step{\textbf{2$_{\bG}$}}
\BeginSelectG{
    $B_{g'} \leftarrow 
    \{b'\in B:~~(b',g')   \in E_t(\om),~(g',b')\not\in E_t(\om)\}$\;
    \eIf{$B_{g'} \neq \emptyset$}{
    		Select $b''$ uniformly at random from $B_{g'}$\;
		}
		{	
			Select $b''$ uniformly at random from $B$\;
		}
}
    \caption{\om~(Oblivious~Online~MatchMaker)}
\end{algorithm}

\begin{algorithm}
	\SetKwBlock{BeginSelectB}{\textbf{$\bullet$ Step 2$_{\bB}$}}{end}
	\SetKwBlock{BeginSelectG}{\textbf{$\bullet$ Step 2$_{\bG}$}}{end}
    \SetKwInOut{Input}{\scriptsize{$\triangleright$ INPUT}}
    \SetKwInOut{Step}{$\bullet$ Step}
    \Input{User sets $B$ and $G$}
    \vspace{0.3cm}
    \textbf{At each round $t$:}\\
    \vspace{0.3cm}%
%    \Step{\textbf{2$_{\bB}$}}
\BeginSelectB{
    $G^+_b\!\!\leftarrow\!\!
    \{g'\in G:(g',b)\in E_{t-1}(\idom),{\color{blue} s(g',b)=1},(b,g')\not\in E_{t-1}(\idom)\}$\;
    \eIf{$G^+_b \neq \emptyset$}{
    		Select $g$ uniformly at random from $G^+_b$\;
		}
		{	
			Select $g$ uniformly at random from $G$\;
		}    
		}
    \vspace{0.3cm}
    %
%    \Step{\textbf{2$_{\bG}$}}
\BeginSelectG{
    $B^+_{g''}\!\!\leftarrow\!\!
    \{b'\in B:(b',g'')\in E_t(\idom),{\color{blue} s(b',{g''})  =1},(g'',b')\not\in E_t(\idom)\}$\;
    \eIf{$B^+_{g''} \neq \emptyset$}{
    		Select $b''$ uniformly at random from $B^+_{g''}$\;
		}
		{	
			Select $b''$ uniformly at random from $B$\;
		}
}
    \caption{\idom~(Information~Driven~Online~MatchMaker)}
\end{algorithm}

During each round, \om\ operates in the following way. When a boy $b$ is selected at step $1_B$, it chooses at step $2_B$ a girl $g$ uniformly at random from the whole set $G$. 
We denote by $B_{g'} \subseteq B$ the subset containing all boys that showed their preference ({\em positive or even negative}) for $g'$ in the previous rounds, while the preference of $g'$ for anyone of them has not been received yet.
When a girl $g'$ is selected at step $1_G$, if $B_{g'}$ is not empty, the algorithm chooses at step $2_G$ a boy uniformly at random from the subset $B_{g'} \subseteq B$.  When $B_{g'}$ is empty, then \om\ selects a boy uniformly at random from the whole set $B$~\footnote{Observe that in this case it could also select more than once the same boy for the same girl $g'$ during the $T$ rounds. The optimality proof for this algorithm implies that this does not significantly affect its performance.}. Interestingly enough, \om\ does {\em not} depend on the edge sign assignment $s$. 

\bigskip

We also describe another algorithm, called \idom\ 
(Information Driven Online MatchMaker), which can be useful as baseline for experimental evaluations. 
Although we do not analyse the performance of \idom, we strongly believe that it outperforms \om\ on real-world datasets. 




\idom\ operates in the following way. \\
During each round $t$, when a boy $b$  
is selected at step $1_B$, \idom\ chooses a girl uniformly at random from the subset $G^+_b \subseteq G$. This subset is formed by the girls which previously {\em showed to like $b$} while the preference of $b$ for them is not known yet during round $t$. When $G^+_b$ is empty, then \idom\ selects a user uniformly at random from the whole set $G$. \idom\ operates in an specular way when selecting a boy at step $2_G$ for the girl selected at step $1_G$, i.e. the behaviour of the algorithm is symmetric w.r.t. the first and last three steps of the online problem protocol. 

%In order to prove the optimality of \idom, we will show another optimal algorithm which can be seen as its simplified version: \om~(Oblivious Online MatchMaker). 

%Even if we prove that both algorithms are in fact optimal up to a constant factor, we strongly believe that \idom~outperforms \om\ on real world datasets, and the ratio of their optimality factors can be significant in the results of an experimental evaluation of their performance [\textit{\color{ForestGreen} \textbf{FV}: This conjecture will be shown in a future experimental evaluation.}]. We see \om~ also as especially useful to prove the lower bound of \idom\ in Theorem~\ref{th:adversarialLB}.

It is not clear yet whether \idom\ is optimal (like \om) or suboptimal. If \idom\ is suboptimal, the reason must be related to the fact it is misled by the edge signs of the input graph. In fact, we can prove that that eliminating 
in the \idom\ pseudocode {\color{blue} $s(g',b)=1$} and {\color{blue} $s(b',g'')=1$} respectively from the condition of step $2_B$ and $2_G$, we obtain another optimal algorithm (it can be seen as a symmetric version of \om, where the first three steps mimic the last three ones; [\textit{\color{ForestGreen} \textbf{FV}: In order to prove this optimality result it is sufficient to extend the proof of Theorem~\ref{th:adversarialLB}}]). 
This fact would show that, in the worst case, the edge sing information can be misleading for any algorithm. However, in real-world scenarios, we believe that \idom\ can take advantage of the edge sign information outperforming \om, and
%[\textit{\color{ForestGreen} \textbf{FV}: This should be formally proven focusing on the input characterization.}] 
this is the main reason we describe this information driven algorithm.


\medskip
%For any given boy $b$, define now $E_b^+$ as the edge set formed by all positive edges incoming to $b$ and define also  
%$E_B^+ \defeq \cup_{b\in B} E_b^+$. Finally, let $R_B^+$ be the set of all edges of $E_B^+$ together with their respective reciprocal edges, i.e. $R_B^+ \defeq E_B^+ \cup \{(g,{g'})  : ({g'},g)   \in E_B^+\}$.
%\medskip
The following 
%two
Lemma plays a crucial role in the proof for the lower bound of the number of matches found by \om.

\begin{lemma}\label{l:soamuar}
$E^r_T(\om)$ is selected {\em uniformly at random} in $E^r$.
\end{lemma}



%\begin{fact}\label{f:oamuar}
%During the whole sequence of $T$ rounds, the pairs of reciprocal edges found by \idom\ at step $2_B$ -- \enquote{if} branch, when $G_b^+$ is not empty, are selected uniformly at random fromrandom from $R_B^+$.
%\end{fact}

  




We now prove the \om\ lower bound.

\begin{theorem}\label{th:adversarialLB}
Given any input graph $\scG(B,G,E,s)$, if $T-n=\Omega(n)$ and $T=\scO(n^2)$, then $\E\, E^r_T(\om)=\Theta(T)$ and the expected number of matches found by 
\om\ satisfies: 
\[
\E M_T(\om)
=\Theta\left(\frac{T}{n^2}M\right)~.
\]
\end{theorem}



==> proof_hammingDistance.tex <==
\subsection{Proof of Lemma~\ref{le:hammingDistance}}
%
\begin{proof}
Let $R_k=\{i_1, i_2, \ldots, i_k\}$.
Let $\scV(A,\bc)$ be the multiset containing all $A$'s column vectors such that, for all $\bv \in \scV(A,\bc)$, the Hamming distance between $\bc$ and $\bv$ is lager than $\frac{\beta r}{k}\log r$. Clearly, we have $|\scV(A,\bc)|\le c$. 
Thus, given any vector $\bv \in \scV(A,\bc)$, the probability that it belongs to $\scA(R_k, \boldsymbol{c})$ can be upper bounded as follows:
%\[
%\Pr(\bv \in \scA(R_k, \bc))=
%\prod_{i \in R_k} \Pr(\bv_{i}=\bc_{i})
%\le \left(1-\frac{\beta\frac{r}{k}\log c}{r}\right)^{|R_k|}\le c^{-\beta+1}~.
%\] 
\begin{align}
\Pr(\bv \in \scA(R_k, \bc))
&=\Pr\left(\bv_{i_j}=\bc_{i_j}~\forall j\in[k]\right)\nonumber\\
&\le
\left(1-\frac{\frac{\beta r}{k}\log r}{r}\right)^{k}\nonumber\\
&=
\left(1-\frac{\beta\log r}{k}\right)^{k}\nonumber\\
%%%+e^{-\frac{k}{8}}\label{eq:cf}\nonumber\\
%&\le %\left(1-r^{1-\beta}\right) 
%r^{-\beta}+r^{-\beta}\nonumber\\
&\le r^{-\beta}\nonumber~.%\label{eq:kbound}~.
\end{align}

%where in inequality~\ref{eq:cf} we applied a Chernoff bound to limit the cardinality of $R_k$ by $k$, and in inequality~\ref{eq:kbound} we 
%used the statement assumption $k\ge \lceil 8 \beta \log r\rceil$.


The probability that there exists at least one vector 
belonging to both $\scV(A,\bc)$ and $\scA(R_k, \bc)$, can be therefore bounded as follows:
\begin{align}
\Pr(|\scV(A,\bc) \cap \scA(R_k, \bc)|\neq \emptyset)
&\le\sum_{\bv \in \scV(A,\bc)}\Pr(\bv \in \scA(R_k, \bc))\label{eq:unionBound}\\
&\le|\scV(A,\bc)|%\,2
\,r^{-\beta}\nonumber\\
&\le %2\,%
c\,r^{-\beta}\nonumber\\
&\le %2\,%
r^{1-\beta}\label{eq:setSize}~,
\end{align}

where in inequality~(\ref{eq:unionBound}) we simply use the Union Bound and in inequality~(\ref{eq:setSize}) we took into account that $|\scV(A,\bc)|\le c \le r$.
\end{proof}


==> proof_urommLB.tex <==
\subsection{Proof of Theorem~\ref{th:urommLB}}
\begin{proof}%\textbf{of Theorem~\ref{th:urommLB}}
~\textit{[Sketch]}.~
The match bound can be simply proven by calculating the probability that, for each match between two users $b$ and $g$, 
both $(b,g)$ and $(g,b)$ belong to $E_T(\uromm)$.
\end{proof}

==> protocol.tex <==
\section{Problem setting and related notation}\label{s:protocol}

In an online fashion
\iffalse
\footnote{\textit{\color{ForestGreen} \textbf{FV}: In the final version of the paper the protocol will consist in three steps solely: during each round \textbf{(i)} the learner receives a user $u$ chosen uniformly at random in $V$, and \textbf{(ii)} is required to select an element $u'$ belonging to $\cV(u)$. 
\textbf{(iii)} The sign of $s(u,u')$ is finally revealed. Using this protocol, the changes in the bounds and the proofs provided in this draft version will be negligible. Note that having a protocol with three steps where, during each round, one boy and one girl will be simultaneously served, would result in oversimplifying the design of the learning algorithm. In fact, this way the learner could verify during each round if two users like each other in one step.}}
\fi
, during each round $t \le T$, \textbf{(i)} the learner receives a boy $b$ chosen uniformly at random from $B$, and \textbf{(ii)} is required to select a girl $g \in G$. 
\textbf{(iii)} The sign of $s(b,g)$
is then revealed. After having received this edge sign information, the  three steps described above are executed using set $G$ in place of $B$ in \textbf{(i)}, and $B$ in place of $G$ in \textbf{(ii)}. These six steps are performed for $T$ rounds in total. In general, we assume $n \le T\le n^2$.


\bigskip

The problem online protocol can be described more formally in 
Figure~\ref{f:protocol}. 

\begin{figure}[!h]
\vspace{0.2cm}
\noindent\rule{9cm}{0.4pt}
\vspace{-0.2cm}
\begin{description} 
\item [Repeat $T$ times:]
\end{description}
\vspace{-0.4cm}
\noindent\rule{9cm}{0.4pt}
\vspace{-0.2cm}
\begin{description} 
\item [\colorbox{white}{1$_{\bB}$}] Receive $b \in B$ (selected uniformly at random from $B$).  
\item [\colorbox{verylightgray}{2$_{\bB}$}] \colorbox{verylightgray}{\textbf{\em Select} $g \in G$.}
\item [\colorbox{white}{3$_{\bB}$}] Receive $s(b,g)$.
\end{description}
\vspace{-0.3cm}
\noindent\rule{9cm}{0.4pt}
\vspace{-0.1cm}
\begin{description}
\item [\colorbox{white}{1$_{\bG}$}] Receive $g' \in G$ (selected uniformly at random from $G$).  
\item [\colorbox{verylightgray}{2$_{\bG}$}] \colorbox{verylightgray}{\textbf{\em Select} $b' \in B$.}
\item [\colorbox{white}{3$_{\bG}$}] Receive $s(g',b')$.
\end{description}
\vspace{-0.4cm}
\noindent\rule{9cm}{0.4pt}
\caption{The online problem protocol. The actions performed by the learner consist only in the user selections of step \colorbox{verylightgray}{$2_B$} and \colorbox{verylightgray}{$2_G$}. The goal is to design a selection strategy maximising the number of {\em matches found}. A {\em match} is defined as a pair of users $b'' \in B$ and $g'' \in G$ such that $s(b'',g'')=s(g'',b'')=1$. The matches {\em found} by the learner are the ones whose edge signs %$s(b'',g'')$ and $s(g'',b'')$
are received at step $3_B$ and $3_G$ respectively (not necessarily during the same round).}\end{figure}\label{f:protocol}

\bigskip


We define a \textbf{{\em match}} as a pair of {\em positive  reciprocal} edges\footnote{Thus, using the matrix notation we have a match between two users $b$ and $g$ iff 
$\bB_{b,g}=\bG_{b,g}=1$.}. We denote by $\scM$ the {\em undirected} graph having $V$ as user set and such that two users are connected by an edge iff they realize a match in $\scG$. We call $\scM$ \enquote{{\em matching graph}}. Thus, the adjacency matrix of $\scM$ can be written as follows: 
\[ \begin{pmatrix}
   \bzero & \bB\circ\bG\\\
(\bB\circ\bG)^{\top} & \bzero
 \end{pmatrix}
 \]
Given $u \in V$, we denote by $\scN_{\scM}(u)$ as the set of nodes adjacent to $u$ in $\scM$. We also denote 
by $\degree_{\scM}(u)$ the degree in $\scM$ of a user $u$.
%the intersection of all the adjacency neighborhood of $u$ and $u'$ in $\scM$. 
Finally, we call {\em uniformly random bipartite graph} any undirected bipartite graph with vertex set partition $\scP=(V_1,V_2)$, where the edge set is generated as follows: For each pair of nodes $u \in V_1$ and $u' \in V_2$, an edge connecting $u$ with $u'$ is created independently with the same probability $p \in [0,1]$.  

The goal of the algorithm is to maximise the number of matches between boys and girls during $T$ rounds. 
%i.e. the number of pairs of signs $s(b,g)  $ and $s(g,b)$ both equal to $1$ that are revealed to the learner during the $T$ rounds, at steps $3_B$ and $3_G$. 
We denote by $M_t(A)$ the number of matches obtained by a given algorithm $A$ after $t$ rounds. Thus, the goal is to design an algorithm $A$ in order to maximise $M_T(A)$. We also denote by $M$ the {\em total} number of matches present in $\scG(B,G,E,s)$. Finally, we define $E_t(A)$ and $E^r_t(A)$ as the set of respectively directed edges and reciprocal directed edges %namely all the pairs of edges $(b,g),(g,b)$, that are 
selected by $A$ during the first $t$ rounds\footnote{We have therefore $E_0(A)=E^r_0(A)=\emptyset$.}. $E^r$ is defined as the set of {\em all} $|B|\cdot|G|=n^2$ pairs of reciprocal edges between $B$ and $G$. %Hence, for any round $t$ and any algorithm $A$, we have $E_t(A) \subseteq E$ and $E^r_t(A) \subseteq E^r$.

 

\bigskip

%The problem can be also defined in terms of {\em preference matrices}. In this case, we would have two $n$ by $n$ matrices, denoted by $B$ and $G$, where each element is either $-1$ or $1$. We would indicate the matrix indices by using $b, i, j, k \in [n]$ for $B$ and $g, u, v, w \in [n]$ for $G$.
%More precisely, $B_{b,g} \in \{-1,1\}$ represents the preference of boy $b$ for girl $g$. 
%Analogously, $G_{{g'},{b'}} \in \{-1,1\}$ represents the preference of boy $b'$ for girl $g$. Thus, a match consists by a boy index $b''$ and a girl index ${g''}$ such that both $B_{b'',{g''}}$ and $G_{{g''},{b''}}$ are equal to $1$, i.e. boy $b''$ and girl ${g''}$ like each other. 


==> refinements.tex <==
\subsection{Model and algorithm refinements}\label{s:refinements}

%What we discussed in the previous subsection is useful to build the main structure of models and matchmakers.
%There is still room for improvements both for the problem modelization and the algorithmic design.

We discuss here some possible improvements both for the problem modelization and the algorithmic design.

\begin{enumerate}
 
\item It would be interesting to 
%formally quantify the tightness of the result of Lemma~\ref{le:nonuniformCC}. This could be very helpful to
refine the bound of Theorem~\ref{th:smileTimeNeeded}, showing to what extent the optimality requirements of the statement of Theorem~\ref{th:smileMatchMequalMstar} are necessary, especially for what concerns the total number of matches $M$. 
 
\item An extension indeed very interesting both from a theoretical and practical perspective, consists in assessing the matchmaker performance while taking into account how \enquote{fast} the users are matched. Formally, we could evaluate the performance of an algorithm $A$ with the sum of $M_t(A)$ over all rounds $t$, i.e.
\[
\sum_{t \in [T]} M_t(A)~,
\]
or, more in general, given two suitably chosen functions $f$ and $g$,
\[
f\left(\sum_{t \in [T]} g(M_t(A))\right)~.
\]
Maximizing this kind of matckmaker performance originates from the need to interleave the matching information collection and its exploitation, with challenging problems of theoretical and practical importance. Since this objective appears to be significant especially in realistic real-world scenarios, it would be also interesting to develop (at least) some heuristic methods drawing inspiration from this performance measure and carrying out an experimental analysis.

\item We could easily extend the model and the algorithms taking into account that the number of boys and girls are different, namely having $|B|=n_B$ and $|G|=n_G$, where the ratio $\frac{n_B}{n_G}$ is constant. We could also have two different number of description categories, namely $C_B$ for boys and $C_G$ for girls. 

\item Another natural extension consists in considering non-binary preferences. We could have an $s$ function from $E$ to $[0,1]$ (or $[-1,1]$), expressing to what extent a boy likes a girl and vice versa. When the codomain of $s$ is $[0,1]$, each pairs reciprocal edges $(b,g)$ and $(g,b)$ would be naturally associated with the reward $s(b,g)\cdot
s(g,b)$. Thus, the adjacency matrix of the matching graph $\scM$, which would be now a {\em weighted} graph, could be represented again as follows:
\[ \begin{pmatrix}
   \bzero & \bB\circ\bG\\\
(\bB\circ\bG)^{\top} & \bzero
 \end{pmatrix}
 \]
The weight of each edge $(u,u')$ of $\scM$ would be therefore $s(u,u')\cdot s(u',u)$ when $V(u)\neq V(u')$. Otherwise it would be null.
In this case a natural way to assess the performance could be represented by the cumulative reward obtained during $T$ rounds. 

\iffalse
\item We defined the description and preference features of 
each user as a pair of $d$-dimensional $0\,$-$1$ binary vectors. However, in this draft we did not exploit yet this user structural characterization. In fact, we just considered each user as having a description feature which can be seen as an integer in $[C]$. The same holds for the preference features associated with each user, which can be represented as $C$-dimensional binary vectors. 
It would be interesting to explore variations of the model exploiting the vectorial feature (hidden) representations. For instance we could introduce a notion of probability of a match between two users $b \in B$ and $g \in G$ proportional to the hamming distance between $\bp(b)$ and $\bd(g)$, and between $\bp(g)$ and $\bd(p)$. Additionally, the elements of the two vectors could be real numbers in $[0,1]$. In this case the probability of a match
between $b$ and $g$ could be proportional to a suitable distance between the two pairs of vectors involved in the match realization. 
\textit{\color{ForestGreen} \textbf{FV} However, I believe this could easily lead to the issues present in Figure~\ref{f:counterexample}, i.e. to a matching graph $\scM$ that is \enquote{similar} to a uniformly random bipartite graph. For instance, independently of $d$, if all users are associated with only two description vectors and two preference vectors, such that the probability of a match for each pair of users is the same, like in Figure~\ref{f:counterexample}, no algorithm can be able to learn which are the matching users.}
\fi

 
\item The protocol could be made more realistic if, at step 
$2_B$ and $2_G$, we had a sequence of selections for serving the same user in place of just one single selection. The length of the sequence could be modelled by a random function which may be always the same, or depending on each single user.
Another possibility for suitably modifying the protocol, would be having a discrete distribution for the user system login, scil. we can associate to each user $u \in V$ a probability $p(u)$ such that $\sum_{u \in V(u)} p(u)=1$, and at the first protocol step the users are selected according to  $p(\cdot)$. Finally, it would be interesting to take into account the possibility of having a dynamic signed network evolving over time, for instance in such a way that at each round some new users can be added to $V$, while some others can be removed. 



\item {\color{ForestGreen} \textbf{FV}: I would now prefer to remove the \idom\ algorithm if you agree.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\item The problem could be extended taking into account the 
most common asymmetries we can have between $B$ and $G$. The number boys and girls can be different. Additionally, the number of boy preference categories/girl description categories can be different from the one of girl preference categories/boy description categories. The same holds for the pair of vectors $\bp(b)$ and $\bd(g)$, and the pair of vectors $\bp(g)$ and $\bd(b)$, for all $b \in B$ and $g \in G$. 

\item Instead of modelling the description and preference features of each user with a pair of $d$-dimensional vectors, we could explore the possibility to replace $\scA_f$ with an assumption based on $P_M(\cdot|\cdot)$ and the exploitation of this probability estimations for all pair of boys and girls. For instance, assume $M=n^{1+\alpha}$ with $\alpha > 1$. We know that if the matching graph $\scM$ is a uniform bipartite graph, in expectation we have
$P_M(b|b')=n^{\alpha/2}$ and $P_M(g|g')=n^{\alpha/2}$ 
for every pairs of distinct boys and distinct girls respectively. Since with such matching graphs it is easy to show there is no efficient learning strategy, we must have, in general, sufficiently large subsets $B_0$ of $B$ where $P_M(b|b')$ is larger than $n^{\alpha/2}$ for all $b,b' \in B_0$ (the same must hold symmetrically for $G$). In fact, this is also the case of the model based on description and preference features, but it is not clear if there exists an assumption strictly more general than $\scA_f$ that allows us to design an efficient matchmaker. 

\item Another quantity that can be useful in designing an efficient matchmaker, could be the following notion of description similarity between any
pair of users. Given any pair of boys $b$ and $b'$, 
we define as $\sigma_{b,b'}$ as the probability that selecting a girl $g$ uniformly at random from $G$, we have $s(g,b)=s(g,b')$. Analogously, given any pair of girls $g$ and $g'$, we define as $\sigma_{g,g'}$ as the probability that selecting a boy $b$ uniformly at random from $B$, we have $s(b,g)=s(b,g')$. 
%Let $S$ be the set formed by all these values.
%The main idea is to design an algorithm able to exploit the estimated values of $P$ and $S$, in order to make a ranking of all girls at step $2_B$ and all boys at step $2_G$ based on the expectation of finding a new match.
It could be very interesting to find a method for obtaining an estimation of the description similarities between any pair of users, in order to spare rounds in the sampling phase. However, in order to obtain such $n$ feedback provided by the girls for even a single boy, we would need 
$\widetilde{\Theta}(n^2)$ rounds because of the protocol. The same symmetrically holds for girls. Hence, we could think to have $\widetilde{\Theta}(n^{\alpha})$ rounds to have for each boys the feedback of $n^{\alpha}$ girls. 
\fi

\end{enumerate}
%===========
\iffalse

%The above described assumption requires, in other words, that for each user $u$ there exists a group of users in the same set ($B$ or $G$), that is \textbf{(i)} not too small, and \textbf{(ii)} formed by users having a positive preference similarity, between them and $u$, which is larger than a threshold $\tau$. 

%We conjecture that if this assumption is satisfied, it is possible to find an expected number of matches which can be expressed in terms of $\beta$ and $\tau$. We also believe there are two constant 
%$\beta^*\in (0,1)$ and $\tau^* \in (0,1)$ such that, when $\beta\ge\beta^*$ and $\tau\ge\tau^*$, this expected number of matches is always equal to $\omega\left(\frac{T}{n^2}M\right)$ making possible to {\em learn}
%the edge sign assignment $s$.


%We model this learning problem by making assumptions that allow to estimate such conditional probabilities
%and exploit them to find new matches.

%\medskip



%\medskip

%Finally, we believe that a significant value for setting $T$ must be both subquadratic and superlinearithmic in $n$, i.e. $T=o(n^2)$ and $T=\omega(n \log n)$. In our online setting, $n^{3/2}$ seems a reasonable value for setting $T$ in order to assess the performance of any given matchmaker.

\fi
%===========
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\appendix

%\newpage

%\section{Main proofs}\label{a:mainproofs}





%\section{Supplementary proofs}\label{a:suppproofs}


%\begin{proof}\textbf{of Fact~\ref{f:oamuar}}.~
%At step $2_B$ of each round, when $G_b^+$ is not empty, the \enquote{if} branch is selected and \idom\ finds a {\em new} pair of reciprocal edges $\{(b,g)  ,(g,$b)\}$ (even if it does not find necessarily a match). 
%Each pair of reciprocal edges found this way is the result of the previous selections of boys which are selected uniformly at random from $B$ (step $2_G$ -- \enquote{else} branch). 
%We also observe that girl $g$ at step $2_B$ is selected uniformly at random from set $G_b^+$, which contains only girls that like boy $b$. Hence, we can conclude that the pairs of reciprocal edges found by \idom\ whenever $G_b^+$ is not empty during the whole sequence of $T$ rounds, are {\em selected uniformly at random} in $R_B^+$. 
%\end{proof}

==> remarkOptimality.tex <==
\subsection{On the optimality of \smi}\label{a:remarkOptimality}

It is worth explaining why, whenever 
$M=\omega\left(n^{3/2}\sqrt{\log n}\right)$, the additive term
$\frac{n^3\log n}{M}$ present in the bound 
$T=\omega\left(n\,(C^G+C^B)+\frac{n^3\log(n)}{M}\right)$
of Corollary~\ref{co:smileMatchMequalMstar}, becomes equal to $o(M)$, while the first term $n\,(C^G+C^B)$ can be upper bounded by 
$n\,(C^G_0+C^B_0)$. In fact, the lower bound on $T$ of Theorem~\ref{th:smileTimeNeeded} to uncover $\Theta(M)$ matches is $T=\Omega(n\,(C^G_0+C^B_0)+M)$. Thus, 
it might appear at first sight quite surprising that, the larger is the number of matches $M$, the smaller becomes the second term in the bound of 
Corollary~\ref{co:smileMatchMequalMstar}, which {\em seemingly} leads to a contradiction.

However, it is important to take into account that in Corollary~\ref{co:smileMatchMequalMstar} $T$ must be large enough to satisfy even the condition $M^*_T=M$ (with high probability). When $M$ is large, the number of rounds necessary to satisfy $M^*_T=M$ becomes much larger than the one needed to satisfy the condition 
$T=\omega\left(n\,(C^G+C^B)+ \frac{n^3\log(n)}{M}\right)$. It is possible to get an insight about this fact especially focusing on the case in which $M$ is large and the term $n(C^G+C^B)$ is small: as intuition suggests, the number of rounds needed by the Omniscent Matchmaker to match $M$ users, which must be equal to $\Omega(M)$, will be larger than $n\,(C^G+C^B)+ \frac{n^3\log(n)}{M}$. In conclusion, if the number of rounds needed by \smi\ to uncover $\Theta(M)$ matches is equal to the one needed by the Omniscent Matchmaker to uncover $M$ matches, then we can state \smi\ is optimal up to a constant factor, because there not exist any algorithm able to outperform the Omniscent Matchmaker.
%In this case the number of rounds used to match the users will be much larger than the one to estimate which users match. 

This provides a crucially important insight into the key factors allowing the additive term $\frac{n^3\log n}{M}$ to be equal to $o(M)$ in Corollary~\ref{co:smileMatchMequalMstar}, which represents in fact one of the main keystones of the proof of 
Theorem~\ref{th:smileMatchMequalMstar}.

==> smilePseudocode.tex <==
\subsection{Pseudocode of procedures Cluster Estimation and User Matching}

In this section, we present the pseudocode of the procedures called by the main body \smi\ pseudocode: Cluster Estimantion and User Matching.

\begin{procedure}[!h]
    \SetKwInOut{Input}{\scriptsize{$\triangleright$ INPUT}}
    \SetKwInOut{Output}{\scriptsize{$\triangleright$ OUTPUT}}
	\SetKwBlock{BeginSelectB}{(2$_B$)}{end}
	\SetKwBlock{BeginSelectG}{(2$_G$)}{end}
    \Input{$B$ and $G$, parameter $S > 0$.}
    \Output{Set of clusters $\scC$, set of feedbacks $\scF$.}
    %%%%%%%%%%%%Build sample sets
    {\bf Init:} 
    \begin{itemize}
    \vspace{-0.2in}
    \item $F_u \gets \emptyset$\ \ $\forall u \in B\cup G$\,; \texttt{/* One set of feedbacks per user $u \in B\cup G$ */}
    \item $B^r\gets \emptyset$; $G^r\gets \emptyset$\,; \texttt{\hspace{0.24in}/* One set of cluster representatives per side
    */}
    \item $r_{u}\gets 0$\ \ $\forall u \in B\cup G$\,; \texttt{/* No user is candidate to belong to $B^r\cup G^r$ */}
    \end{itemize}
    %$B(g,S) \gets \emptyset$;~~~~
    %~~~~
    %\textbf{foreach} $b \in B$ \textbf{do}
    %$G(b,S) \gets \emptyset$;~~~~
    %$F(b) \gets \emptyset$\;
    Let $G=\{g_{1},\ldots, g_{n}\}$,~~~~$B=\{b_{1},\ldots, b_{n}\}$,~~~~$S'\defeq 2S+4\sqrt{S\log n}$, ~~~~ $i,j \gets 1$;\\
    %\While{$(|F(g_{n})|<\frac{n}{2}~\vee~g_n)~\wedge~(|F(b_{n})|<\frac{n}{2}~\vee~b_n\not\in B_S)$}{
    At each round $t$\,:\\
    \eIf{$i\le n~\vee~j\le n$}{
	\BeginSelectB{
	Let $b \in B$ be the boy selected in Step ($1_B$);\\
	\eIf{$i \le n$}{
	Select $g_i$;~~~~$F_{g_i}\gets F_{g_i}\cup\{b\}$\;
	\If{$|F_{g_i}|= S'\wedge r_{g_i}=0$}{\texttt{/* Try to assign $g_i$ to some cluster based on $G^r$ */\\ } 
	\eIf{$\exists g^r \in G^r\, :\, \forall b'\in F_{g_i}\cap F_{g^r}~~s(b',g_i)=s(b',g^r)$}{Set $\ctg(g_i)=g^r$;~~~$i\gets i+1$;
	}{\texttt{/* $g_i$ will be included into $G^r$ as soon as $|F_{g_i}|=\frac{n}{2}$ */\\ } $r_{g_i}\gets 1$\;}
	}
	\texttt{/* If $g_i$ is a cluster representative */}\\
	\If{$|F_{g_i}|=\frac{n}{2}$}{$G^r \gets G^r\cup \{g_i\}$;~~$i\gets i+1$;} 
}{
	Select $g \in G$ arbitrarily;
}
}
	\BeginSelectG{Do the same as in Step (2$_B$) after switching $B$ with $G$, $b$ with $g$, $B_r$ with $G^r$, $i$ with $j$, etc.}
}
{Set:~ $\ctg(g^r) = g^r~~\forall g^r \in G^r$;~~~ $\scC \gets \cup_{u\in B\cup G}\{(u,\ctg(u))\}$;~~~ $\scF \gets \cup_{u\in B\cup G}\{(u,F_u)\}$\;
\Return{$(\scC,\scF)$~.}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%Return results 
    \caption{Cluster Estimation() -- \smi~(Phase I)}	 
\end{procedure}

\bigskip

\begin{procedure}[!h]
    \SetKwInOut{Input}{\scriptsize{$\triangleright$ INPUT}}
    \SetKwInOut{Output}{\scriptsize{$\triangleright$ OUTPUT}}
	\SetKwBlock{BeginSelectB}{\textbf{(2$_{\bB}$)}}{end}
	\SetKwBlock{BeginSelectG}{\textbf{(2$_{\bG}$)}}{end}
	\Input{$B$ and $G$, set of clusters $\scC$, set of feedbacks $\scF$.}
	At each round $t$\,:\\
		\BeginSelectB{
		\textit{Let $b \in B$ the boy selected in Step ($1_B$);}\\
		\eIf{$\exists g \in G : b\in F(\ctg(g)) \wedge g\in F(\ctg(b)) \wedge s(b,\ctg(g)) = s(g,\ctg(b))=1 \wedge (b,g)\not\in E_t(\smi)$}{select $g$\;}{
   		select $g\in G$ arbitrarily\;}}
		\BeginSelectG{
		Do the same as in Step (2$_B$) after switching $B$ with $G$, and $b$ with $g$.
	}
    \caption{User Matching() -- \smi~(Phase II)}
\end{procedure}

